Preference-CFR$\:$ Beyond Nash Equilibrium for Better Game Strategies

Artificial intelligence (AI) has surpassed top human players in a variety of games. In imperfect information games, these achievements have primarily been driven by Counterfactual Regret Minimization (CFR) and its variants for computing Nash equilibrium. However, most existing research has focused on maximizing payoff, while largely neglecting the importance of strategic diversity and the need for varied play styles, thereby limiting AI's adaptability to different user preferences. To address this gap, we propose Preference-CFR (Pref-CFR), a novel method that incorporates two key parameters: preference degree and vulnerability degree. These parameters enable the AI to adjust its strategic distribution within an acceptable performance loss threshold, thereby enhancing its adaptability to a wider range of strategic demands. In our experiments with Texas Hold'em, Pref-CFR successfully trained Aggressive and Loose Passive styles that not only match original CFR-based strategies in performance but also display clearly distinct behavioral patterns. Notably, for certain hand scenarios, Pref-CFR produces strategies that diverge significantly from both conventional expert heuristics and original CFR outputs, potentially offering novel insights for professional players.

==> PZ.tex <==
%! Author = juqi
%! Date = 2025/1/30

% Preamble
Although a NE strategy can yield the best payoff in a worst-case scenario,
it often does not align with people's expectations.
Consider the following choices: first, to receive \$4,500 with 100\% certainty;
second, to have a 50\% chance of winning \$10,000,
but also a 50\% chance of winning nothing.
While the expected payoff of the second option is higher,
most people prefer the guaranteed \$4,500.
This preference stems from the fact that,
compared to the potential risk, losing \$500 is within a tolerable range.

